Synthesizing Environment-Specific People in Photographs

We present ESP, a novel method for context-aware full-body generation, that enables photo-realistic synthesis and inpainting of people wearing clothing that is semantically appropriate for the scene depicted in an input photograph. ESP is conditioned on a 2D pose and contextual cues that are extracted from the photograph of the scene and integrated into the generation process, where the clothing is modeled explicitly with human parsing masks (HPM). Generated HPMs are used as tight guiding masks for inpainting, such that no changes are made to the original background. Our models are trained on a dataset containing a set of in-the-wild photographs of people covering a wide range of different environments. The method is analyzed quantitatively and qualitatively, and we show that ESP outperforms the state-of-the-art on the task of contextual full-body generation.

==> tab/tab-fid-kid.tex <==

\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
     \textbf{Method}  & \textbf{$\beta=0$} & \textbf{$\beta=0.25$} & \textbf{$\beta=0.5$} & \textbf{$\beta=0.75$} & \textbf{$\beta=1$} \\
        %
    \midrule
     Baseline & - &  - & 78.7 & 86.7 & 90.0  \\
        %
     \textbf{Ours} & 42.3 & 22.6 & 21.0 & \textbf{19.8} & 20.2  \\
        %
    \bottomrule
    \end{tabular}
}
\caption{\textbf{ControlNet Strength:} the table shows FID$\downarrow$ scores for varying $\beta$ across 10K images. Our method outperforms SOTA.}

\label{tab:beta}
\end{table}



==> tab/tab_fixed.tex <==

\begin{table}
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{crccccc}
    \toprule
     \textbf{C} & \textbf{Evaluation}  & PSNR $\uparrow$& MSE $\downarrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & KID $\downarrow$\\
    \midrule
     & HPM  & \textbf{20.44}&\textbf{0.0102} & \textbf{0.051}  & \textbf{11.5} & \textbf{0.0098} \\
    
     F & Blurry Context & \textbf{23.33} & \textbf{0.0060} & \textbf{0.123} & \textbf{41.1} & 0.0412\\
    
     & Real Context & \textbf{21.94} & \textbf{0.0078} & \textbf{0.154} & - & - \\
    
    \midrule
     & HPM  & 20.37 & 0.0104 & 0.053  & 12.2 & 0.0104 \\
    
     R & Blurry Context & 11.81 & 0.0769 & 0.361 &  41.4 & \textbf{0.0389}\\
    
     & Real Context & 11.71 & 0.0781 & 0.358 & - & - \\
    
    \midrule
     F & VAE Recon.  & 27.05 & 0.0022 & 0.051 & 7.0 & 0.0029 \\
    
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Quantitative Analysis:} the results are calculated over 10K contexts. C denotes whether the context vector is fixed (F) or random (R). Overall, fixing the context vector leads to predictions that are closer to the ground truth, especially in background reconstruction. Therefore, the analysis confirms that our method is context-aware (PSNR, MSE, LPIPS) and generates meaningful parsing masks and background contexts (FID, KID). The performance of the standalone VAE module used to generate the blurry contexts (rows 2 and 5) is shown in the last row.}

\label{tab:fixed}
\end{table}



==> tab/tab_psi.tex <==

\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
     \textbf{Output} & \textbf{$\psi=0.5$}  & \textbf{$\psi=0.6$} & \textbf{$\psi=0.7$} & \textbf{$\psi=0.8$} & \textbf{$\psi=0.9$} & \textbf{$\psi=1$} \\

    \midrule
     HPM & 15.73 &  14.59 & 13.53 & 12.64 & 11.96 & \textbf{11.49} \\


     Context & 112.45 &  86.33 & 67.55 & 54.77 & 46.29 & \textbf{41.08} \\
    
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Truncation Trick:} the table shows FID$\downarrow$ scores for varying $\psi$ across 10K randomly selected contexts. The optimal value of $\psi$ is equal to $1.0$ for both the HPM and the Context generator.}

\label{tab:psi}
\end{table}


